LEGO: Leveraging Experience in Roadmap Generation for Sampling-Based Planning

We consider the problem of leveraging prior experience to generate roadmaps in sampling-based motion planning. A desirable roadmap is one that is sparse, allowing for fast search, with nodes spread out at key locations such that a low-cost feasible path exists. An increasingly popular approach is to learn a distribution of nodes that would produce such a roadmap. State-of-the-art is to train a conditional variational auto-encoder (CVAE) on the prior dataset with the shortest paths as target input. While this is quite effective on many problems, we show it can fail in the face of complex obstacle configurations or mismatch between training and testing. We present an algorithm LEGO that addresses these issues by training the CVAE with target samples that satisfy two important criteria. Firstly, these samples belong only to bottleneck regions along near-optimal paths that are otherwise difficult-to-sample with a uniform sampler. Secondly, these samples are spread out across diverse regions to maximize the likelihood of a feasible path existing. We formally define these properties and prove performance guarantees for LEGO. We extensively evaluate LEGO on a range of planning problems, including robot arm planning, and report significant gains over heuristics as well as learned baselines.

==> figs/diverse_bottleneck_experiment_results.tex <==
% !TEX root = ../main.tex

\begin{figure*}[!ht]
\centering
  \begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig_bottleneck/shortest}
    \caption{}
    \label{fig:bottleneck_sp}     
    \vspace*{1em}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig_bottleneck/bottleneck}
    \caption{}
    \label{fig:bottleneck_bottleneck}     
    \vspace*{1em}
  \end{subfigure}
  \hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig_diverse/shortest}
    \caption{}
    \label{fig:diverse_sp}     
    \vspace*{1em}
  \end{subfigure}  
  \hfill
  \begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig_diverse/diverse}
    \caption{}
    \label{fig:diverse_diverse}     
    \vspace*{1em}
  \end{subfigure}
\caption{(a) and (b) compare the samples generated by \algSP and \algBottleneck respectively. 
(c) and (d) compare the samples generated by \algSP and \algDiversity respectively. In both instances, \algSP fails to find a solution.}
\label{fig:bd_experiments}
% \vspace{-6mm}
\end{figure*}

==> figs/experiment_results.tex <==
% !TEX root = ../main.tex

\begin{figure*}[!ht]
\centering
%   \begin{subfigure}[b]{0.27\textwidth}
%     \centering
%     \includegraphics[height=9.56em]{fig_bottleneck/bottleneck_success_rate}
%     \caption{}
%     \label{fig:bottleneck_success_rate}
%     \vspace*{1em}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.27\textwidth}
%     \centering
%     \includegraphics[height=9.56em]{fig_bottleneck/bottleneck_path_length}
%     \caption{}
%     \label{fig:bottleneck_path_length}     
%     \vspace*{1em}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.21\textwidth}
%     \centering
%     \includegraphics[height=8.6em]{fig_bottleneck/shortest}
%     \caption{}
%     \label{fig:bottleneck_shortest_example}     
%     \vspace*{1em}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.21\textwidth}
%     \centering
%     \includegraphics[height=8.6em]{fig_bottleneck/bottleneck}
%     \caption{}
%     \label{fig:bottleneck_bottleneck_example}     
%     \vspace*{1em}
%   \end{subfigure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \begin{subfigure}[b]{0.27\textwidth}
%     \centering
%     \includegraphics[height=9.56em]{fig_diverse/diverse_success_rate}
%     \caption{}
%     \label{fig:diverse_success_rate}
%     \vspace*{1em}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.27\textwidth}
%     \centering
%     \includegraphics[height=9.56em]{fig_diverse/diverse_path_length}
%     \caption{}
%     \label{fig:diverse_path_length}     
%     \vspace*{1em}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.21\textwidth}
%     \centering
%     \includegraphics[height=8.6em]{fig_diverse/shortest}
%     \caption{}
%     \label{fig:diverse_shortest_example}     
%     \vspace*{1em}
%   \end{subfigure}  
%   \begin{subfigure}[b]{0.21\textwidth}
%     \centering
%     \includegraphics[height=8.6em]{fig_diverse/diverse}
%     \caption{}
%     \label{fig:diverse_diverse_example}     
%     \vspace*{1em}
%   \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    \includegraphics[height=9.56em]{fig_lego/lego_success_rate}
    \caption{}
    \label{fig:4_2D_sr}
  \end{subfigure}
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    \includegraphics[height=9.56em]{fig_lego/lego_path_length}
    \caption{}
    \label{fig:4_2D_pl}     
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=8.6em]{fig4/fig4_c}
    \caption{}
    \label{fig:4_2D_sp}     
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=8.6em]{fig4/fig4_d}
    \caption{}
    \label{fig:4_2D_lego}     
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \includegraphics[height=9.56em]{fig_n_link_arm/sr}
    \caption{}
    \label{fig:4_3D_sr}
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \includegraphics[height=9.56em]{fig_n_link_arm/pl}
    \caption{}
    \label{fig:4_3D_pl}
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=8.6em]{fig_n_link_arm/sp}
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \caption{}
    \label{fig:4_3D_sp}     
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=8.6em]{fig_n_link_arm/lego}
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \caption{}
    \label{fig:4_3D_lego}     
    \vspace*{1em}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \includegraphics[height=9.56em]{fig4/fig4_e}
    \caption{}
    \label{fig:4_3D_sr}
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \includegraphics[height=9.56em]{fig4/fig4_f}
    \caption{}
    \label{fig:4_3D_pl}
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=8.6em]{fig_snake/SP_3L}
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \caption{}
    \label{fig:4_3D_sp}     
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=8.6em]{fig_snake/LEGO_3L}
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \caption{}
    \label{fig:4_3D_lego}     
    \vspace*{1em}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    \includegraphics[height=8.6em]{fig_herb/herb_success_rate}
    \caption{}
    \label{fig:4_herb_sr}
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    \includegraphics[height=8.6em]{fig_herb/herb_path_length}
    \caption{}
    \label{fig:4_herb_pl}     
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[trim=50 20 30 0, clip, height=8.6em]{fig_herb/herb_sp}
    \caption{}
    \label{fig:4_herb_sp}     
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[trim=0 20 50 0, clip, height=8.6em]{fig_herb/herb_lego}
    \caption{}
    \label{fig:4_herb_lego}
    \vspace*{1em}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Comparisons of \algSP against \algLEGO. Each row follows pattern (from the left): First figure shows the success rate, second figure shows the normalized path length, third figure shows \algSP and fourth figure shows \algLEGO.}
\label{fig:experiments}
\end{figure*}

==> figs/suppl_experiment_results.tex <==
% !TEX root = ../supplementary.tex

\begin{figure*}[!ht]
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 2D POINT ROBOT
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    \includegraphics[height=10.70em]{fig_lego/lego_success_rate}
    \caption{}
    \label{fig:4_2D_sr}
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    \includegraphics[height=10.70em]{fig_lego/lego_path_length}
    \caption{}
    \label{fig:4_2D_pl}     
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig4/fig4_c}
    \caption{}
    \label{fig:4_2D_sp}     
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig4/fig4_d}
    \caption{}
    \label{fig:4_2D_lego}     
    \vspace*{1em}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 5D SNAKE
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \includegraphics[height=10.70em]{fig4/fig4_e}
    \caption{}
    \label{fig:4_3D_sr}
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \includegraphics[height=10.70em]{fig4/fig4_f}
    \caption{}
    \label{fig:4_3D_pl}
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig_snake/SP_3L}
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \caption{}
    \label{fig:4_3D_sp}     
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig_snake/LEGO_3L}
    % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
    \caption{}
    \label{fig:4_3D_lego}     
    \vspace*{1em}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 9D SNAKE
  % \begin{subfigure}[b]{0.27\textwidth}
  %   \centering
  %   % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
  %   \includegraphics[height=10.70em]{fig4/fig4_e}
  %   \caption{}
  %   \label{fig:4_7D_sr}
  %   \vspace*{1em}
  % \end{subfigure}
  % \begin{subfigure}[b]{0.27\textwidth}
  %   \centering
  %   % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
  %   \includegraphics[height=10.70em]{fig4/fig4_f}
  %   \caption{}
  %   \label{fig:4_7D_pl}
  %   \vspace*{1em}
  % \end{subfigure}
  % \begin{subfigure}[b]{0.21\textwidth}
  %   \centering
  %   \includegraphics[height=10.75em]{fig_snake/SP_3L}
  %   % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
  %   \caption{}
  %   \label{fig:4_7D_sp}     
  %   \vspace*{1em}
  % \end{subfigure}
  % \begin{subfigure}[b]{0.21\textwidth}
  %   \centering
  %   \includegraphics[height=10.75em]{fig_snake/LEGO_3L}
  %   % \framebox[\linewidth]{\raisebox{0pt}[0.7\linewidth][0pt]{{\large Snake}}}
  %   \caption{}
  %   \label{fig:4_7D_lego}     
  %   \vspace*{1em}
  % \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig_herb/herb_success_rate}
    \caption{}
    \label{fig:4_herb_sr}
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.27\textwidth}
    \centering
    \includegraphics[height=10.75em]{fig_herb/herb_path_length}
    \caption{}
    \label{fig:4_herb_pl}     
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[trim=50 20 30 0, clip, height=10.75em]{fig_herb/herb_sp}
    \caption{}
    \label{fig:4_herb_sp}     
    \vspace*{1em}
  \end{subfigure}
  \begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[trim=0 20 50 0, clip, height=10.75em]{fig_herb/herb_lego}
    \caption{}
    \label{fig:4_herb_lego}
    \vspace*{1em}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Comparisons of \algSP against \algLEGO. Each row follows pattern (from the left): First figure shows the success rate, second figure shows the normalized path length, third figure shows \algSP and fourth figure shows \algLEGO.}
\label{fig:experiments}
\end{figure*}

==> inputs/approach.tex <==


\section{Approach}
\label{sec:approach}

% In this section, we present \algLEGO (Learning Efficient Graph Oracles), an algorithm for training a CVAE with a key subset of nodes that can be used to generate a sparse, high quality roadmap. It consists of two main components inspired by the two shortcomings identified in~\sref{sec:shortest_path}. Firstly, we identify \emph{bottleneck nodes} on the dense graph. These are nodes that are essential to ensure the predicted roadmap contains a near optimal solution. Secondly, we identify a \emph{diverse pathset}. \scnote{This segue sucks. Need a crisper intro.} 

In this section, we present \algLEGO (Leveraging Experience with Graph Oracles), an algorithm to produce the training input for the CVAE. We address the challenges identified in~\sref{sec:framework}. Firstly, we recognize that it is often too difficult for the learner to directly predict the shortest path. Instead, we train it to predict only \emph{bottleneck nodes} that can assist the underlying search in finding a near-optimal solution. Secondly, the test data may contain unexpected obstacles. We safeguard against this by training the learner to predict a \emph{diverse set of paths} with the assumption that one of them is feasible. 

\begin{algorithm}[t]
  \caption{ \algLEGO }\label{alg:lego_node_generation}
  \algorithmStyle
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}

  \Input{ Planning problem $\pp$, \\ \ Dense graph $\denseGraph$, Sparse graph $\sparseGraph$}
  \Output{ \algLEGO nodes $\vertexSetLEGO$}

  $\vertexSetLEGO \gets \emptyset$\; 
  $\PathSetDiv \gets \algDiversity(\pp, \denseGraph)$\label{line:lego:diversity}\;
  \For{$\Path \in \PathSetDiv$}
  {
    $\vertexSetBN \gets \algBottleneck(\pp, \Path, \sparseGraph)$\label{line:lego:bottleneck}\;
    $\vertexSetLEGO \gets \vertexSetLEGO \cup \vertexSetBN$ 
  }
  \Return{$\vertexSetLEGO$}\;
\end{algorithm}

Algorithm~\ref{alg:lego_node_generation} describes a high level pseudo-code of \algLEGO. We first find a set of diverse paths on the dense graph (Line~\ref{line:lego:diversity}). 
We then iterate over each path and extract bottleneck nodes for this path (Line~\ref{line:lego:bottleneck}). These bottleneck nodes from the diverse paths are then used as input to the CVAE to learn a sampling distribution (Section~\ref{sec:framework}). This is illustrated in \figref{fig:cvae_input}. We now describe how bottleneck nodes and diverse paths are computed. Detailed algorithms and proofs are provided in~\cite{vernwal2018roadmaps}.

\subsection{Bottleneck Nodes}
\label{sec:approach:bottleneck}

We begin by noting that $\sparseGraph$ has a sparse but uniform coverage over the entire configuration space. Hence, the learner only has to contribute a critical set of nodes that allow $\sparseGraph$ to represent paths that are near-optimal with respect to a path $\densePath$ generated from a dense graph. We call these \emph{bottleneck nodes}. The name indicates that these are difficult-to-sample nodes, absent in the sparse graph, which are otherwise required to approximate $\densePath$. We define $\inputBottleneck = \algBottleneck(\pp, \denseGraph)$ as:

\begin{definition}[Bottleneck Nodes]
\label{def:bottleneck_nodes}
Given a path on a dense graph $\densePath$, find the smallest set of nodes which in conjunction with a sparse subgraph $\sparseGraph$ contains a near-optimal path, i.e.
\begin{equation}
\small
\label{eq:bottleneck_nodes}
\begin{aligned}
\argmin_{\vertexSet \subset \densePath} & & & \abs{\vertexSet} \\
\text{s.t.} & & & \cost(\alg( \sparseGraph \compose \vertexSet , \pp)) \leq (1 + \epsilon)\cost(\densePath)  
\end{aligned}
\end{equation}
\end{definition}


\begin{algorithm}[t]
  \caption{ \algBottleneck }\label{alg:bottleneck_node_generation}
  \algorithmStyle
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}

  \Input{ Planning problem $\pp$, \\ \ Dense path $\densePath$, Sparse graph $\sparseGraph$}
  \Output{ Bottleneck nodes $\vertexSetBN$}

%  $\densePath^* \gets \alg(\denseGraph, \pp)$ \label{line:bn:dense_sol} \Comment*[r]{Shortest dense path}
  $\inflatedGraph \gets \sparseGraph \compose \densePath$, $\eta \gets 1$ \;\label{line:bn:compose} 
  \While{$ \cost(\alg( \inflatedGraph , \pp)) \leq (1 + \epsilon) \cost(\densePath ) $ \label{line:bn:iteration_start}}
  {
    $\eta \gets \eta + \delta \eta$ \;\label{line:bn:inflate} 
    Inflate by $\eta$ the weight of edges $\edge \in \inflatedEdgeSet \setminus \sparseEdgeSet$ \label{line:bn:iteration_end}\;
  }
  $\vertexSetBN \gets \densePath \cap \alg( \inflatedGraph , \pp)$ \;
  \Return{$\vertexSetBN$}\;
\end{algorithm}

\setlength{\textfloatsep}{10pt}

This optimization (\ref{eq:bottleneck_nodes}) is combinatorially hard. We present an approximate solution in Algorithm~\ref{alg:bottleneck_node_generation}. We begin by creating a composed graph $\sparseGraph \compose \densePath$ (Line~\ref{line:bn:compose}). We inflate weights of newly added edges by $\inflation$ (Line~\ref{line:bn:inflate}) to disincentivize the search from using any of the newly added edges. This inflation factor is increased till a near-optimal path can no longer be found (Lines~\ref{line:bn:iteration_start}-\ref{line:bn:iteration_end}). At this point, the additional vertices that the shortest path on this inflated path passes through are essential to achieve near-optimality, i.e. are the bottleneck nodes. This is formalized by the following guarantee:

\begin{proposition}[Bounded bottleneck edge weights]
Let $\edgeSetBN \gets \inflatedPath^* \setminus \sparseEdgeSet$ be the chosen bottleneck edges, $\edgeSetBN^*$ be the optimal bottleneck edges and $\densePath^*$ be the optimal path on $\denseGraph$.
\begin{equation}
\sum_{\edge_i \in \edgeSetBN} \weight(\edge_i) \leq \sum_{\edge_i \in \edgeSetBN^*} \weight(\edge_i) + \frac{(1 + \epsilon) \cost(\densePath^*)}{\inflation}
\end{equation}
\end{proposition}

\figref{fig:bd_experiments} illustrates the samples generated by (a) \algSP{} and (b) \algLEGO{} trained with samples from \algBottleneck{}; and the successful routing through narrow passages using samples from \algLEGO.

\subsection{Diverse PathSet}
\label{sec:approach:diversity}

In this training scheme, we try to ensure the roadmap is \emph{robust} to various sources of errors such as the test world contains unexpected obstacles or that the feature vector does not catpure sufficient details of the world. One antidote to this process is \emph{diversity} of samples. Specifically, we want the roadmap to have enough diversity such that if the predicted shortest path is in fact infeasible, there are low cost alternates. 

We set this up as a two player game between a planner and an adversary. The role of the adversary is to invalidate as many shortest paths on the dense graph $\denseGraph$ as possible with a fixed budget of edges that it is allowed to invalidate. The role of the planner is to find the shortest feasible path on the invalidated graph and add this to the set of diverse paths $\PathSetDiv$. The function $\inputDiversity = \algDiversity(\pp, \denseGraph)$ then returns nodes belonging to $\PathSetDiv$. We formalize this as:

\begin{definition}[Diverse PathSet]
\label{def:diverse_path_set}
 We begin with a graph $\graph^0 = \denseGraph$. At each round  $i$ of the game, the adversary chooses a set of edges to invalidate:
\begin{equation}
\label{eq:cover_ksp}
\edgeSet^*_i = \argmaxprob{\edgeSet_i \subset \edgeSet, \abs{\edgeSet_i} \leq \ell} \cost(\alg( \graph^{i-1} \remove \edgeSet_i , \pp))  
\end{equation}
and the graph is updated $\graph^i = \graph^{i-1} \remove \edgeSet^*_i$. The planner choose the shortest path $\Path_i = \alg( \graph^{i} , \pp))$ which is added to the set of diverse paths $\PathSetDiv$. 
\end{definition}

The optimization problem~\eref{eq:cover_ksp} is similar to a set cover problem (NP-Hard~\citep{feige1998threshold}) where the goal is to select edges to cover (invalidate) as many paths as possible. If we knew the exact set of paths to cover, it is well known that a greedy algorithm will choose a near-optimal set of edges~\citep{feige1998threshold}. We have the inverse problem - we do not know how many consecutive shortest paths can be covered with a budget of $\ell$ edges. 

\begin{algorithm}[t]
  \caption{ \algDiversity }\label{alg:diverse_pathset_generation}
  \algorithmStyle
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}

  \Input{ Planning problem $\pp$, \\ \ Dense graph $\denseGraph$, Sparse graph $\sparseGraph$}
  \Output{ Diverse pathset $\PathSetDiv$}

  $\PathSet \gets \alg^{L}( \denseGraph , \pp)$ \label{line:div:ksp}  \Comment*[r]{L-shortest paths}
  \For{$i = 1, \cdots, k$}
  {
    $\edgeSet_i \gets \emptyset$\;
    \While{ $\abs{\edgeSet_i} < \ell$}
    {
      Add the next $\ell - \abs{\edgeSet_i}$ paths from $\PathSet$ to $\PathSet$\label{line:div:succ}\;
      $\edgeSet_i \gets \textsc{SetCover}(\PathSetInv)$\;\label{line:div:set_cover}
    }
    Add the next path from $\PathSet$ to $\PathSetDiv$\;
  } 
\Return{$\PathSetDiv$}\;
\end{algorithm}

Algorithm~\ref{alg:diverse_pathset_generation} describes the procedure. We first compute a large set of shortest feasible paths (Line~\ref{line:div:ksp}). The adversary successive paths to eliminate till it runs out of budget (Line~\ref{line:div:succ}). It then runs greedy set cover on these paths to see if they can be eliminated with a smaller budget (Line~\ref{line:div:set_cover}). If so, the process continues till the set cover exhausts the budget. Hence at termination, we ensure:
\begin{proposition}[Near-optimal Invalidated EdgeSet]
Let $\PathSetInv$ be the contiguous set of shortest paths invalidated by Algorithm~\ref{alg:diverse_pathset_generation} using a budget of $\ell$. Let $\ell^*$ be the size of the optimal set of edges that could have invalidated $\PathSetInv$.
\begin{equation}
\ell \leq (1 + \log \abs{\PathSetInv}) \ell^*
\end{equation}
\end{proposition}
\figref{fig:bd_experiments} illustrates the samples generated by (a) \algSP{} and (b) \algLEGO trained with samples from \algDiversity{}; and the robustness to unexpected obstacles exhibited by \algLEGO{}.


\begin{figure}[!t]
\centering
  \begin{subfigure}[b]{0.24\columnwidth}
    \centering
    \includegraphics[height=6.1em]{fig_bottleneck/shortest}
    \caption{}
    \label{fig:bottleneck_sp}     
    \vspace*{1em}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.24\columnwidth}
    \centering
    \includegraphics[height=6.1em]{fig_bottleneck/bottleneck}
    \caption{}
    \label{fig:bottleneck_bottleneck}     
    \vspace*{1em}
  \end{subfigure}
  \hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[b]{0.24\columnwidth}
    \centering
    \includegraphics[height=6.1em]{fig_diverse/shortest}
    \caption{}
    \label{fig:diverse_sp}     
    \vspace*{1em}
  \end{subfigure}  
  \hfill
  \begin{subfigure}[b]{0.24\columnwidth}
    \centering
    \includegraphics[height=6.1em]{fig_diverse/diverse}
    \caption{}
    \label{fig:diverse_diverse}     
    \vspace*{1em}
  \end{subfigure}
\caption{Comparison of samples (distribution illustrated as heatmap) generated by \algSP{} (a, c) and \algDiversity{} (b, d) in different environments. In the first environment (left), \algLEGO{} (b) is trained with samples from \algBottleneck{}. In the second environment (right), \algLEGO{} (d) is trained with samples from \algDiversity{}. In both instances, \algSP fails to find a solution.}

% Sample distributions generated by \algSP{} (a, c) and \algLEGO{} (b, d) in different environments.

% (a) and (c) illustrate the samples generated by \algSP in different environments. They are compared to samples generated by \algLEGO{} when trained on samples from (b) \algBottleneck{} and (d) \algDiversity{}. In both instances, \algSP fails to find a solution.}
\label{fig:bd_experiments}
% \vspace{-6mm}
\end{figure}



==> inputs/framework.tex <==


\section{Framework}
\label{sec:framework}

We now present a framework for training graph predicting oracles as illustrated in \figref{fig:overall_framework}(a). This is a generalization of the approach presented in \cite{ichter2017learning}. The framework applies three main approximations. First, instead of predicting a subgraph $\graph \subset \denseGraph$, we learn a mapping that directly predicts states $\state \in \stateSpace$ in continuous space.\footnote{For cases where a subgraph is preferred, e.g. $\denseGraph$ lies on a constraint manifold, one can design a projection operator $\mathcal{P} : \stateSpace \rightarrow \denseVertexSet$} Secondly, instead of solving a structured prediction problem, we learn an i.i.d sampler that will be invoked repeatedly to get a set of vertices. These vertices are then connected according to an underlying connection rule, such as $k$-NN, to create a graph. Thirdly, we compose the sampled graph with a \emph{constant sparse graph} $\sparseGraph \subset \denseGraph, \abs{\sparseGraph} \leq N$. This ensures that the final predicted graph has some minimal coverage. \footnote{Since $\denseGraph$ is a Halton graph, we use the first $N$ Halton sequences.} 

The core component of the framework is a Conditional Variational Auto-encoder (CVAE)~\cite{sohn2015learning} which is used for approximating the desired sample distribution. CVAE is an extension of a traditional variational auto-encoder~\cite{kingma2013auto} which is a directed graphical model with low-dimensional Gaussian latent variables. CVAE is a \emph{conditional} graphical model which makes it relevant for our application where conditioning variables are features of the planning problem. We provide a high level description for brevity, and refer the reader to~\cite{vernwal2018roadmaps} for more details and~\cite{doersch2016tutorial} for a comprehensive tutorial.

Here $\state \in \stateSpace$ is the output random variable, $\latentVar \in \real^\latentDim$ is the latent random variable and $\condVar \in \real^\featDim$ is the conditioning variable. We wish to learn two \emph{deterministic mappings} - an \emph{encoder} and a \emph{decoder}. An encoder maps $(\stateVar, \condVar)$ to a mean and variance of a Gaussian $\encoder(\latentVar | \stateVar, \condVar)$ in latent space, such that it is ``close'' to an isotropic Gaussian $\Normal(0, I)$. The decoder maps this Gaussian and $y$ to a distribution in the output space $\decoder(\stateVar | \latentVar, \condVar)$. This is achieved by maximizing the following objective $\loss \left( \stateVar, \condVar; \decoderParam, \encoderParam \right)$:
\begin{equation}
\label{eq:cvae_loss}
	  -D_{KL}\left( \encoder(\latentVar | \stateVar, \condVar) \, || \, \Normal(0, I) \right) + \frac{1}{\latentDim} \sum_{l=1}^{\latentDim} \log \decoder(\stateVar | \condVar, \latentVar^{(l)})
\end{equation}
Note that the encoder is needed only for training. At test time, only the decoder is used to map samples from an isotropic Guassian in the latent space to samples in the output space.

We train the CVAE by passing in a dataset $\dataSet = \{ \stateSetVar_i, \feat_i \}_{i=1}^{D}$. $\feat_i$ is the feature vector (conditioning variable) extracted from the planning problem $\pp_i$. $\stateSetVar_i$ is the desired set of nodes extracted from the dense graph $\denseGraph$ that we want our learner to predict. Hence we train the model by maximizing the following objective. 
\begin{equation}
	\risk(\dataSet; \decoderParam, \encoderParam) = \frac{1}{\abs{\dataSet}} \sum_{i=1}^{\abs{\dataSet}} \sum_{j=1}^{\abs{\stateSetVar_i}} \loss \left( \stateVar_j, \condVar_i; \decoderParam, \encoderParam \right)
\end{equation}

To summarize, the overall training framework is as follows:
\begin{enumerate}
	\item Load a database of planning problems $\pp_i$ and corresponding feature vectors $\feat_i$.
	\item For each $\pp_i$, extract relevant nodes from the dense graph $\denseGraph$ by invoking $\stateSetVar_i = \algAbstract(\pp_i, \denseGraph)$.
	\item Feed dataset $\dataSet = \{ \stateSetVar_i, \feat_i \}_{i=1}^D$ as input to CVAE.
	\item Train CVAE and return learned decoder $\decoder(\stateVar | \condVar, \latentVar)$.
\end{enumerate}

At test time, given a planning problem $\pp$, the graph predicting oracle $\policy(\denseGraph, \feat)$ performs the following set of steps:
\begin{enumerate}
	\item Extract feature vector $\feat$ from planning problem $\pp$.
	\item Sample $N$ nodes using decoder $\decoder(\stateVar | \condVar, \latentVar)$.
	\item Connect nodes to create a graph $\graph$. Compose sampled graph with a constant sparse graph $\graph \leftarrow \graph \compose \sparseGraph$. 
\end{enumerate}

The focus of this work is on examining variants of the the node extraction function $\stateSetVar = \algAbstract(\pp, \denseGraph)$. While the parameters of the CVAE are certainly relevant (which we investigate in~\cite{vernwal2018roadmaps}), in this paper we ask the question:
\begin{quote}
What is a good input $\stateSetVar$ to provide to the CVAE?
\end{quote}
To that end, we explore the following schemes:
\begin{enumerate}
	\item \algSP: Extract nodes $\inputSP$ belonging to the shortest path. This is the baseline approach (\sref{sec:shortest_path}).
	\item \algBottleneck: Extract nodes $\inputBottleneck$ that correspond to bottlenecks along the shortest path (\sref{sec:approach:bottleneck}).
	\item \algDiversity: Extract nodes $\inputDiversity$ belonging to multiple diverse shortest paths (\sref{sec:approach:diversity}).
	\item \algLEGO: Extract nodes $\inputLEGO$ that correspond to bottlenecks along multiple diverse diverse shortest paths. This is our proposed approach (\sref{sec:approach:lego}).
\end{enumerate}



==> inputs/new_framework.tex <==


\section{Framework for Predicting Roadmaps}
\label{sec:framework}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{cvae_input.pdf}
    \caption{%
    \label{fig:cvae_input}
    (a) The training input generated by \algSP. (b) Failure of \algSP model to route through gaps (c) Another failure of the model due to unexpected obstacles (d) The training input generated by \algLEGO. Diverse shortest paths are generated followed by extraction of bottleneck nodes. \fullFigGap
    }
\end{figure*}%

We now present a framework for training graph predicting oracles as shown in \figref{fig:overall_framework}. The framework applies three main approximations. First, instead of predicting a subgraph $\graph \subset \denseGraph$, we train a Conditional Variational Auto-encoder (CVAE)~\citep{sohn2015learning} to approximate a sampling distribution of nodes $\state \in \stateSpace$ in continuous space. Second, instead of solving a structured prediction problem, we learn an i.i.d sampler that will be invoked repeatedly to get a set of vertices. These vertices are then used to construct a graph. Thirdly, we compose the sampled graph with a \emph{constant sparse graph} $\sparseGraph \subset \denseGraph, \abs{\sparseGraph} \leq \abs{\denseGraph{}}$. This ensures that the final predicted graph has some minimal coverage. Refer to~\citep{vernwal2018roadmaps} for details.

\subsection{General train and test procedure}

\paragraph{Training Procedure} At train time \figref{fig:overall_framework}(a), we first load a pair of planning problem $\pp_i$ and feature $\feat_i$. We obtain the target nodes $\stateSetVar_i = \algAbstract(\pp_i, \denseGraph)$. We then feed the dataset $\dataSet = \{ \stateSetVar_i, \feat_i \}_{i=1}^D$ as input to CVAE. Finally, we train the CVAE and return the learned decoder $\decoder(\stateVar | \condVar, \latentVar)$.

\paragraph{Testing Procedure} At test time \figref{fig:overall_framework}(b), we extract feature vector $\feat$ from planning problem $\pp$. We then sample a set $\vertexSet$ of $N$ nodes using decoder $\decoder(\stateVar | \condVar, \latentVar)$. Finally, we create a composed graph $\graph \leftarrow \sparseGraph \compose \vertexSet$. 

The focus of this work is to examine the function $\stateSetVar = \algAbstract(\pp, \denseGraph)$. We ask the question:
\begin{quote}
What is a good input $\stateSetVar$ to provide to the CVAE?
\end{quote}

\subsection{The \algSP (\citet{ichter2017learning}) procedure}

We briefly examine the scheme of training to predict nodes on the shortest path\cite{ichter2017learning} as shown in \figref{fig:cvae_input}. Formally, let $\inputSP = \algSP(\pp, \denseGraph)$ denote the set of nodes belonging to the shortest path returned by $\alg(\denseGraph, \pp)$. The rationality for this scheme is that the distribution of states belonging to the shortest path might lie on a manifold that can be captured by the latent space of the CVAE. If \emph{prediction is perfect}, then indeed this is the optimal solution to Problem.~\ref{prob:optimal_subgraph}. 

% \begin{figure}[!t]
% \centering
%   \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[height=10em]{fig3/fig3_2}
%     \caption{\label{fig:shortest_path_issues_first}}
%   \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[height=10em]{fig3/fig3_3}
%     \caption{\label{fig:shortest_path_issues_second}}
%   \end{subfigure}
% \caption{
% \avknote{Replace this with heatmap + graph visualization?}
% Failure instances of using \algSP. (a) The model gets stuck between routing through the gap and trying to be on the straight line joining start and goal. (b) The model samples through the obstacles since it is not captured in the feature vector. \fullFigGap}
% \label{fig:diverse}
% \end{figure}

After extensive evaluations of the \algSP scheme, we were able to identify two modes of vulnerabilities: 
\begin{enumerate}
	\item \emph{Failure to route through gaps}: \figref{fig:cvae_input}(b) shows the output of the CVAE when there is a gap through which the search has to route to get to the goal. The model gets stuck in a poor local minimum between linearly interpolating start-goal and routing through the gap since the network is not expressive enough to map the feature vector to such a path. This is tantamount to burdening the sampler to solve the planning problem. 
	\item \emph{Presence of unexpected obstacles in test data}: \figref{fig:cvae_input}(c) shows the output of the CVAE when there are small, unexpected obstacles in the test data which were not present in the training data. The learned distribution samples over this obstacle as the model only predicts what could have been the shortest path in the absence of such obstacles. Even if we were to have such examples in the training data, unless the feature extractor detects such obstacles, the problem remains.
\end{enumerate}



==> inputs/results.tex <==


\section{Experimental Results}
\label{sec:results}

In this section we evaluate the performance of \algLEGO on various problem domains and compare it against other samplers. 
We consider samplers that do not assume offline computation or learning such as Medial-Axis PRM (\algMAPRM) \cite{wilmarth1999maprm, holleman2000framework},~Randomized Bridge Sampler (\algRBB)~\cite{hsu2003bridge}, Workspace Importance Sampler (\algWIS{})~\cite{kurniawati2004workspace}, a Gaussian sampler, \algGaussian{} \cite{boor1999gaussian}, and a uniform Halton sequence sampler, \algHalton{} \cite{Hal60}. 
Additionally, we also compare our framework against the state-of-the-art learned sampler \algSP \cite{ichter2018robot} upon which our work is based.

\paragraph{Evaluation Procedure}
For a given sampler and a planning problem, we invoke the sampler to generate a fixed number of samples. 
We then evaluate the performance of the samplers on three metrics: a) sampling time b) success rate in solving shortest path problem and c) the quality of the solution obtained, on the graph constructed with the generated samples. 
%We expect a good sampler to generate high quality samples in less time, and enable construction of graphs that have higher probability of existence of a low-cost solution path.

\paragraph{Problem Domains}
To evaluate the samplers, we consider a spectrum of problem domains.
%ranging across varied simulated environments involving point robots ($\real^2$), n-link arms ($\real^3$, $\real^7$), snake robots ($\real^5,~\real^9$) and on high dimensional manipulation problems involving a 7-DoF robot ($\real^7,~\real^8$). 
The $\real^2$ problems have random rectilinear walls with random narrow passages (Fig. \ref{fig:experiments}(a)). These passages can be small, medium or large in width. The n-link arms are a set of $n$ line-segments fixed to a base moving in an uniform obstacle field (Fig. \ref{fig:experiments}(b)). The n-link snakes are arms with a free base moving through random rectilinear walls with passages (Fig. \ref{fig:experiments}(c)). Finally, the manipulator problem has a 7DoF robot arm~\citep{Srinivasa_2012_7081} manipulating a stick in an environment with varying clutter (Fig. \ref{fig:experiments}(d)). Two variants are considered - constrained ($\real^7$), when the stick is welded to the hand, and unconstrained, when the stick can slide along the hand ($\real^8$). 

\input{figs/time_table}
\input{figs/table}
%\input{figs/diverse_bottleneck_experiment_results}

\paragraph{Experiment Details}
For the learned samplers \algSP and \algLEGO, we use $4000$ training worlds and $100$ test worlds. Dense graph is an $r-$disc Halton graph~\citep{janson2015deterministic}: $2000$ vertices in $\real^2$ to $30,000$ vertices in $\real^8$. 
The CVAE was implemented in TensorFlow~\cite{tensorflow2015-whitepaper} with 2 dense layers of 512 units each.
Input to the CVAE is a vector encoding source and target locations and an occupancy grid. Training time over 4000 examples ranged from 20 minutes in $\real^2$ to 60 minutes in $\real^8$ problems. At test time, we time-out samplers after $5$ sec. The code is open sourced\footnote{\url{https://github.com/personalrobotics/lego}} with more details in \cite{vernwal2018roadmaps}.
%During test time, for \algRBB and \algSP, the split between constant sparse graph and informed samples is $50-50$ across all environments while for $\algLEGO$ the corresponding split is $70-30$ for $\real^2$ problems and $60-40$ for the rest. For each of the planning instances we consider a timeout of 5 seconds for the total time.
%The algorithms considered in this section have all been implemented in Python and simulations run on a Unix system with 2.0GHz CPU and an Intel i3-5005U processor. The specifics are in the publicly available source code: \url{https://github.com/personalrobotics/lego}.

\subsection{Performance Analysis}

\paragraph{Sampling time}
Table~\ref{tab:timing_results} reports the average time each sampler takes for $200$ samples across $100$ test instances. \algSP and \algLEGO are the fastest. \algMAPRM and \algRBB both rely on heavy computation with multiple collision checking steps. \algWIS, by tetrahedralizing the workspace and identifying narrow passages, is relatively faster but slower than the learners. Unfortunately, some of the baselines time-out on manipulator planning problem due to expense of collision checking. 

% , by tetrahedralizing the workspace and identifying the narrow passages, generates useful samples much faster than \algRBB and \algMAPRM but slower than the learned samplers since the workspace preprocessing happens online. \algSP and \algLEGO learn the sampling strategy offline and thus are characterized by low sampling times given a planning environment during test time.

\paragraph{Success Rate}

Table~\ref{tab:benchmark_results} reports the success rates ($95\%$ confidence intervals) on $100$ test instances when sampling $500$ vertices. Success rate is the fraction of problems for which the search found a feasible solution. \algLEGO has the highest success rate. The baselines are competitive in $\real^2$, but suffer for higher dimensional problems. 
% obtained when using different sampling algorithms. Success rate is the fraction of problems for which the search found a feasible solution. We report results for planning over roadmaps with $500$ vertices in each of the environments described above. Owing to their performance observed in Table \ref{tab:benchmark_results}, we compare in \figref{fig:experiments}, the learned samplers \algSP and \algLEGO in their success rates as a function of the number of samples generated.
\paragraph{Normalized Path Cost}
This is the ratio of cost of the computed solution w.r.t. the cost of the solution on the dense graph. Fig.~\ref{fig:experiments} shows the normalized cost for \algHalton, \algSP and \algLEGO - these were the only baselines that consistently had bounded $95\%$ confidence intervals (i.e. when success rate is $\geq 60\%$). \algSP has the lowest cost, however \algLEGO is within $10\%$ bound of the optimal. 

% We report normalized path costs when the $95\%$ C.I. are bounded (i.e. when success rate is $\geq 60\%$). From Table~\ref{tab:benchmark_results}, we note that only \algSP and \algLEGO consistently exhibit at least 60\% success rate and hence compare the two algorithms in Fig.~\ref{fig:experiments}.
% represented by the cost of the path on $\sparseGraph$, constructed using a sampler, normalized with respect to solution on the $\denseGraph$. We report normalized path costs when the $95\%$ C.I. are bounded (i.e. when success rate is $\geq 60\%$). From Table \ref{tab:benchmark_results}, we note that only \algSP and \algLEGO consistently exhibit at least 60\% success rate and hence compare the two algorithms in Fig. \ref{fig:experiments}.

\input{figs/heuristic_baseline}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{experiment_compact.pdf}
    \caption{%
    \label{fig:experiments}
    Comparisons of \algSP against \algLEGO on different problem domains. In each problem domain (column), success rate (top), normalized path lengths (middle) and solutions determined on the roadmaps constructed using samples generated by the two samplers (bottom) are shown. 
    }
\end{figure*}%

\input{figs/mismatch_result}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Observations}
We report on some key observations from Table~\ref{tab:benchmark_results} and \figref{fig:experiments}.
\begin{observation}
\algLEGO consistently outperforms all baselines
\end{observation}\vspace{-0.5em}
As shown in Table~\ref{tab:benchmark_results}, \algLEGO has the best success rate (for $500$ samples) on all datasets. 
The second row in~\figref{fig:experiments} shows that \algLEGO is within $10\%$ bound of the optimal path.
\begin{observation}
\algLEGO places samples only in regions where the optimal path may pass.
\end{observation}\vspace{-0.5em}
\figref{fig:baselines} shows samples generated by various baseline algorithms on a 2D problem. The heuristic baselines use various strategies to identify important regions - \algMAPRM finds medial axes, \algRBB finds bridge points, \algGaussian samples around obstacles, \algWIS divides up space non-uniformly and samples accordingly. However, these methods places samples everywhere irrespective of the query. \algSP takes the query into account but fails to find the gaps. \algLEGO does a combination of both -- it finds the right gaps.
\begin{observation}
\algLEGO has a higher performance gain on harder problems (narrow passages) as it focuses on bottlenecks.
\end{observation}\vspace{-0.5em}
Table~\ref{tab:benchmark_results} shows how success rates vary in 2D problems with small / medium / large gaps. As the gaps gets narrower, \algLEGO outperforms more dominantly. The \algBottleneck component in \algLEGO seeks the bottleneck regions (\figref{fig:bottleneck_bottleneck}).

For manipulator planning $\real^8$ problems, when stick is unconstrained, \algLEGO and \algSP are almost identical. We attribute this to such problems being easier, i.e. the shortest path simply slides the stick out of the way and plans to the goal. When the stick is constrained, \algLEGO does far better. \figref{fig:experiments}(d) shows that \algLEGO is able to sample around the table while \algSP cannot find this path. 
% Table~\ref{tab:benchmark_results} shows that \algLEGO and \algSP are comparable for unconstrained $\real^8$ problems. Upon closer examination, we attribute this to such problems being easier, i.e. the shortest path simply slides the stick out of the way and plans to the goal.

% \figref{fig:4_herb_sp} shows \algSP on a constrained $\real^8$ problem where the stick cannot move in the robot's hand. It is unable to sample around the table and reach the goal. On the other hand, \figref{fig:4_herb_lego} shows a few key samples from \algLEGO which guide the arm around the table. \figref{fig:4_herb_sr} shows that \algLEGO has a better success rate. Note that both learning algorithm significantly outperform \algHalton.
\begin{observation}
\algLEGO is robust to a certain degree of train-test mismatch as it encourages diversity. 
\end{observation}\vspace{-0.5em}
\figref{fig:mismatch_result} shows the success rate of learners on a 2D test environment that has been corrupted. Environment 1 is less corrupted than environment 2. \figref{fig:mismatch_result}(a) shows that on environment 1, \algLEGO is still the best sampler. \algSP (\figref{fig:mismatch_result}(c)) ignores the corruption in the environment and fails. \algLEGO (\figref{fig:mismatch_result}(d)) still finds the correct bottleneck. \figref{fig:mismatch_result}(b) shows that all learners are worse than \algHalton. \algSP(\figref{fig:mismatch_result}(e)) densifies around a particular constrained region while \algLEGO(\figref{fig:mismatch_result}(e)) still finds a path due to the \algDiversity component sampling in multiple bottleneck regions. 
% \begin{observation}
% \algSP finds the shortest path on problems where it does succeed.
% \end{observation}\vspace{-0.5em}
% \figref{fig:baselines} shows th

% \begin{observation}
% \algLEGO is comparable to \algSP for unconstrained $\real^8$ problems.
% \end{observation}\vspace{-0.5em}

% \begin{observation}
% \algLEGO outperforms \algSP for constrained $\real^8$ problems.
% \end{observation}\vspace{-0.5em}

% \subsection{Analysis of \algBottleneck and \algDiversity} 
% In \figref{fig:bd_experiments} we present the qualitative performance of the foundational algorithms of \algLEGO, \algBottleneck and \algDiversity when compared to \algSP, in addressing the vulnerabilities of \algSP mentioned in \sref{sec:framework}. We make the following observations:
%  \begin{observation}
%  \algBottleneck outperforms \algSP in successfully routing the search through narrow passages.
%  \end{observation}
%  % \figref{fig:bottleneck_success_rate} shows that on a $\real^2$ world, \algBottleneck has a significantly higher success rate that \algSP, almost converging to $1.0$ by $400$ samples. \figref{fig:bottleneck_path_length} shows that in terms of path length, \algSP is initially better but both are eventually comparable. This is expected because of the near-optimality objective of \algBottleneck~\eref{eq:bottleneck_nodes}. 

% \figref{fig:bottleneck_sp} shows the \algSP model struggles to find the gap (as discussed in \sref{sec:framework}). \figref{fig:bottleneck_bottleneck} shows that the \algBottleneck model simply has to identify the correct narrow passages.

%  \begin{observation}
%  \algDiversity is robust to train-test mismatch
%  \end{observation}

%  \figref{fig:diverse_sp} shows failure of \algSP on a $\real^2$ world when there are unexpected obstacles. \figref{fig:diverse_diverse} shows how \algDiversity samples in both homotopy classes and hence finds a solution.
% %\figref{fig:diverse_success_rate} shows that \algDiversity has a better success rate. \figref{fig:diverse_path_length} shows that while both algorithms are comparable in terms of path length, \algDiversity has a smaller variance.


==> inputs/revision.tex <==


\section*{Revision}
\label{sec:revision}

\fontsize{10}{12}\selectfont

We thank all reviewers for their thoughtful feedback and comments. 

Our paper provides an algorithm, \algLEGO~(\sref{sec:framework}), to leverage prior experience to bias sampling for roadmap generation. Our method builds upon prior work \cite{ichter2017learning} in training a CVAE in two significant ways
\begin{enumerate}
\item Instead of training with nodes on the shortest path, we train with nodes belonging to a diverse path set that is robust to train-test mismatch (\sref{sec:approach:diversity})
\item Instead of selecting all the nodes belonging to the shortest path, we target bottleneck nodes that are difficult for a uniform low-dispersion sampler to reach. (\sref{sec:approach:bottleneck})
\end{enumerate}
As pointed out by all three reviewers, our findings are insightful and interesting. Based on their insights and concerns, we revise our presentation.

\subsection{Summary of changes}
\paragraph{Experiments} Broadened the scope of experiments and strengthened the analysis.
\begin{enumerate}
\item In Section \ref{sec:results}, we added comparisons of our work against samplers from the medial-axis planning paradigm, \algMAPRM \cite{wilmarth1999maprm, holleman2000framework} and workspace-guided planners, \algWIS \cite{kurniawati2004workspace}, both of which, in addition to \algRBB \cite{hsu2003bridge}, are non-uniform samplers that are conditioned on the planning environment.
\item Additionally, we also introduced two new planning problems in $\real^5$ and $\real^9$ to exhibit the generality of our framework across a range of planning problems and domains. (\sref{sec:results})
\item Table \ref{tab:timing_results} reporting the time taken by each sampling algorithm to generate set number of samples has been added. This provides a comparison over an additional metric alongside success rates and solution quality (Table \ref{tab:benchmark_results}).
\item We restructure \sref{sec:results} to highlight that \algLEGO fundamentally addresses issues with complex environments with narrow passages (Fig. \ref{fig:bottleneck_sp}, \ref{fig:bottleneck_bottleneck}) and encountering test environments that deviate from the training data (Fig. \ref{fig:diverse_sp}, \ref{fig:diverse_diverse}) before comparing the framework to competing sampling techniques. We also make corrresponding observations O1 and O2.

\end{enumerate}

\paragraph{Modified presentation} Revised the preliminary sections.
\begin{enumerate}
\item We simplified the exposition of \sref{sec:introduction} and \sref{sec:framework} placing more emphasis on the key insight behind our work. 
\item We restructure \figref{fig:overall_framework} in similar spirit.
\item More focus has been placed in distinguishing our work from \cite{ichter2017learning}. We introduced a subsection B in \sref{sec:framework} and \figref{fig:cvae_input} to better convey the vulnerabilities that can potentially effect the performance of the work and how \algLEGO can address them.
\end{enumerate}

\paragraph{Additional Details in the Supplementary \cite{vernwal2018roadmaps}}
\begin{enumerate}
\item Further analysis of the parameters governing the CVAE have been added to the supplementary for a better understanding of the choice of parameters and their effect on the performance of the sampler.
\item The supplementary has been enriched with further details regarding the experiments and the implementation of \algLEGO.
\end{enumerate}

\paragraph{Miscellaneous}
\begin{enumerate}
\item Improved the study of related works (\sref{sec:relatedWork}) and broadened the key areas considered within planning and learning fields.
\item Revised figures for improved clarity. (Fig. \ref{fig:intro}, \ref{fig:bd_experiments})
\end{enumerate}

We now address the major concerns and comments from each of the reviewers.

\subsection{Reviewer 1:}

% \begin{quote}
``\emph{Training is an important pre-computation step, and compute times for this phase must be given.}''
% \end{quote}

We acknowledge that learning-based methods shift the major computatitonal expense offline during training and it is important to consider the cost of training. We report the training times for the planning domains considered in \sref{sec:results}.

% \begin{quote}
``\emph{The limits of how similar training and testing environments must be are not explored}''
% \end{quote}

Our work is based on the central tenet that taking advantage of structural similarity of the environment can be useful in generating high quality samples. Our new title now resonates with this key insight that drives our work.

However, we do note that deviation from training examples is a possibility given a test planning instance. We address this as one of the key vulnerabilities of \cite{ichter2017learning}, one of the major issues that we set out to solve in our work. To this end, we introduce the \algDiversity (\sref{sec:approach:diversity}) that enables the algorithm to generate samples along multiple diverse simple paths. This ensures that, when the test environment deviates from the training examples in the presence of unmodelled obstacles or environment features, the algorithm is still robust in generating high quality useful samples.

We present the analysis of the performance of \algDiversity in Fig. \ref{fig:diverse_sp}, \ref{fig:diverse_diverse}. In addition, we also compare \algDiversity against \algSP over the metrics of success rate and solution quality when the test environments vary from training examples in \cite{vernwal2018roadmaps}.

Given that, however, as any other learning-based algorithm, \algLEGO{}’s learned samples would also not be appropriately applicable when the test environments are extremely dissimilar to the training examples. Although this issue can be overcome with additional samples drawn from a non-adaptive sampler like Halton, we agree that in the face of arbitrary dissimilarity, a learned model can falter.

``\emph{The presentation of related work is lacking in key areas}''

We broaden the areas and works we considered to appropriately place our work amongst its peers. To this end, we consider more algorithms from the medial-axis planning paradigm \cite{wilmarth1999maprm, amato1998obprm} and workspace-guided samplers \cite{kurniawati2004workspace}. Additionally, we also acknowledge works presented more recently \cite{kuo2018deep} that solve issues closely related to those addressed by our work with varied approaches.

\subsection{Reviewer 2}

``\emph{Given the existence of the Ichter et al paper, this submission must be rewritten to include a comparison of their methods with Ichter’s.}'' 

Our work is primarily motivated by \cite{ichter2017learning}. To place more emphasis on the distinguishing aspects of our work with Ichter’s, we introduce a new subsection B in \sref{sec:framework} and \figref{fig:cvae_input} in the revised draft. In this section and the accompanying figures Fig. \ref{fig:cvae_input}, \ref{fig:bd_experiments}, we highlight the vulnerabilities in Ichter’s that can potentially effect the sampler and they ways in which \algLEGO addresses these concerns. 

Through sections 4 and 5, we now attempt to emphasize that the major distinguishing component of our work from Ichter’s is in our training step. While Ichter’s work trains the sampler only on the shortest path in a planning instance, in \algLEGO we identify the key bottleneck regions (\sref{sec:approach:bottleneck}) and the multiple diverse simple paths (\sref{sec:approach:diversity}) that exist in the environment to be robust to train-test mismatch.

Moreover, in evaluating our algorithm against competing techniques, we now first compare the performance of our framework’s fundamental building-block-algorithms, \algBottleneck and \algDiversity against Ichter’s. In \figref{fig:experiments}, we also compare the two algorithms over their performance in solution quality and success rates for a given number of samples. We make a similar comparison of Ichter's work with \algBottleneck and \algDiversity independently but we moved it to the supplementary~\cite{vernwal2018roadmaps} for ease of exposition of the main presentation.

\subsection{Reviewer 3}

``\emph{The algorithms and contributed pieces rely heavily on understanding the deep inner workings of the prior CVAE approach}''

We agree that the paper inherits a lot of details from Ichter’s work that we found difficult to convey within the limited space. We reworded \sref{sec:framework} to abstract away the CVAE and instead regard it as a noisy reconstruction of the target input.
 
We have also expanded on details in the supplementary document~\cite{vernwal2018roadmaps}. The supplementary also contains proofs and additional experimental details that help shed light on the process for training models. 

``\emph{The authors only present comparison with non-adaptive approaches}''

We acknowledge the reviewer’s concern in our presentation and therefore introduced comparisons against adaptive sampling techniques: one from medial-axis planning paradigm - \algMAPRM \cite{wilmarth1999maprm} and one from workspace guided planning - \algWIS \cite{kurniawati2004workspace}. 

This is in addition to \algRBB~\cite{hsu2003bridge} and \algSP~\cite{ichter2017learning} that our original exposition compared our algorithm to.

``\emph{The authors only present success rate for the planner. The time required for training and planning, and the quality of the solutions is meaningful as well}''
 
As the reviewer suggests, different samplers can indeed take varied amounts of time to generate high quality of samples. To address this concern and consider sampling time as a metric, we introduce Table \ref{tab:timing_results}. In this table, we report the average time taken by each of the sampling algorithms to generate a fixed number of samples (200), in each of the planning domains, across 100 planning instances.

In addition to the tables, through the plots in \figref{fig:experiments}, we compare the solution quality or path lengths returned by Ichter's \algSP and \algLEGO, the two learned samplers in our suite of sampling algorithms. In Fig. \ref{fig:intro}, \ref{fig:bd_experiments} we also present a qualitative comparison in the roadmaps generated by \algSP and \algLEGO and its components (\algDiversity, \algBottleneck).

We also report the time taken for training the learned samplers in Section ref[]. 

``\emph{Experimental analysis - the experimental analysis is very basic}''

To strengthen and perform a more rigorous experimental analysis, we introduce a new planning domain that is parameterizable in its dimensionality. We consider an N-Link planar snake robot modelled as a series of links with revolute joints. Additionally the robot’s base link position has two degrees-of-freedom making it an N+2 DoF system. We implement the sampling algorithms on 3-link (5DoF) and 7-link (9 DoF) snake robots in 2D environments with narrow passages. With this new planning domain, we now perform our analyses across a range of planning domains with varying dimensionality ($\real^2$, $\real^5$, $\real^7$, $\real^8$ and $\real^9$) including real robot planning problems in $\real^7$ (constrained) and $\real^8$ (unconstrained).

Moreover, we also expand our analyses to now include sampling time as a metric. As noted by the reviewer and as described above, we also introduce comparison against other adaptive approaches to better place our algorithm amongst competing methods.



==> inputs/shortest_path_issues.tex <==


\section{Shortcomings of Encoding the Shortest Path}
\label{sec:shortest_path}

We examine the scheme applied in~\cite{ichter2017learning} of using nodes belonging to the shortest path on the dense graph as input for training the CVAE. Formally, let $\inputSP = \algSP(\pp, \denseGraph)$ denote the set of nodes belonging to the path returned by $\alg(\denseGraph, \pp)$. The rationality for this scheme is that the distribution of states belonging to the shortest path might lie on a manifold that can be captured by the latent space of the CVAE. This hypothesis is validated across many high-dimensional planning domains. 

We argue that the presented results should not be entirely surprising. The intrinsic difficulty of a planning problem stems from having to search in multiple potential homotopy classes to find a feasible high quality solution. This often manifests in problems involving mazes, bugtraps or narrow passages where the search has to explore and backtrack frequently. Simply increasing the dimension of the problem does not necessarily render it difficult. On the contrary, since the volume of free space increases substantially, there is often an abundance of feasible paths. The challenge, of course, is to find a manifold on which such paths lie with high probability. This is where we found the CVAE to be critical - it learns to \emph{interpolate} between the start and goal along a low dimensional manifold. We validate this observation on real world manipulation problems in~\cite{vernwal2018roadmaps}. 

\begin{figure}[!t]
\centering
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[height=10em]{fig3/fig3_2}
    \caption{\label{fig:shortest_path_issues_first}}
  \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[height=10em]{fig3/fig3_3}
    \caption{\label{fig:shortest_path_issues_second}}
  \end{subfigure}
\caption{Failure instances of using \algSP. (a) The model, which tries to interpolate between start and goal, is unable to deviate enough to sample through the gap. (b) Since the unexpected obstacle does not appear in the feature vector, the model samples in the wrong gap}
\label{fig:diverse}
\end{figure}


However, we are interested in more \emph{difficult} problems where such interpolations would break down. Based on extensive evaluations of this \algSP scheme, we were able to identify two concrete vulnerabilities: 
\begin{enumerate}
	\item \emph{Significant Deviations through Gaps}: \figref{fig:shortest_path_issues_first} shows the output of the CVAE when there is a gap through which the search has to route in order to get to the goal. The learned distribution, which is an interpolation between start and goal, is not flexible enough to sample points along such a path. The root cause of this problem is that the CVAE is unable to find a direct mapping from the feature vector to a manifold on which this path would lie. In this case, such a mapping is almost as challenging as the original search problem.
	% \item \emph{Multiple Narrow Passages}: \figref{fig:shortest_path_issues}(a) shows the output of the CVAE when there are multiple narrow passages that are spatially spread out. The learned distribution samples states in the regions spanning these gaps, even though these samples are highly unlikely to belong to the optimal path. The root cause of this problem is that the latent space is a unimodal Gaussian distribution. Since the decoder is a continuous mapping, this implies that the predicted samples will form a \emph{connected component}. 
	\item \emph{Presence of Unexpected Obstacles}: \figref{fig:shortest_path_issues_second} shows the output of the CVAE when there are small, undetected obstacles in the environment. Undetected implies the obstacles are not captured in the feature vector. The learned distribution samples over this obstacle as it interpolates start and goal. This vulnerability arises from training only using the shortest path. This is a legitimate issue as the feature vector will always be a compressed representation of the planning problem. Having full information requires a high dimension feature vector to be populated by densely probing the environment at all locations before any planning can begin. This also requires an exponential increase in training data that covers all possible configurations in which obstacles can appear.
\end{enumerate}


==> macros.tex <==

% Caligraphic letters:
\newcommand{\calA}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\calC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\calE}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\calG}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\calR}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\calM}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\calX}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\calS}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}\xspace}
\newcommand{\calT}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\calL}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\calB}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\calW}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\calV}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\calP}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\calD}{\ensuremath{\mathcal{D}}\xspace}

% math
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\D}{\mathbb{D}}


\newcommand{\ch}{\mathrm{ch}}
\newcommand\norm[1]{\left\lVert#1\right\rVert}


% Motion planning
\newcommand{\Cfree}{\ensuremath{\calX_{\rm free}}\xspace}
\newcommand{\Cforb}{\ensuremath{\calX_{\rm forb}}\xspace}
%\newcommand{\Csafe}{\ensuremath{\calX_{\rm free}^{\rm safe}}\xspace}
\newcommand{\Crisk}{\ensuremath{\calX_{\rm risk}}\xspace}
\newcommand{\Csafe}{\ensuremath{\calX_{\rm safe}}\xspace}

% Data Structures
\newcommand{\Qfront}{\ensuremath{\calQ_{\rm frontier}}\xspace}
\newcommand{\Qupdate}{\ensuremath{\calQ_{\rm update}}\xspace}
\newcommand{\Qextend}{\ensuremath{\calQ_{\rm extend}}\xspace}
\newcommand{\Qrewire}{\ensuremath{\calQ_{\rm rewire}}\xspace}
\newcommand{\Srewire}{\ensuremath{\calS_{\rm rewire}}\xspace}



%\def\len#1{\ensuremath{{{\rm len}(#1)}}}
%\def\len#1{\ensuremath{\lvert #1 \rvert }}
\def\len#1{\ensuremath{w(#1)}}
\def\llen#1{\ensuremath{\hat{w} (#1)}}


\newcommand{\ab}{\algname{LRA*}}
\newcommand{\ione}{\ensuremath {\infty / 1}- {\text{Lazy Dijkstra}}\xspace}
\newcommand{\ib}{\ensuremath {\infty / \beta}- {\text{Lazy Dijkstra}}\xspace}


\newcommand{\vs}{\ensuremath v_{\rm source}}
\newcommand{\vg}{\ensuremath v_{\rm target}}

\newcommand{\SP}{\calS\calP}


\newcommand{\DOF}{\textit{dof}\xspace}
\newcommand{\DOFs}{\textit{dofs}\xspace}

% =
\newcommand{\eg}{{e.g.}\xspace}
\newcommand{\ie}{{i.e.}\xspace}
\newcommand{\etc}{{etc.}\xspace}
\newcommand{\etal}{{et~al.}\xspace}

\def\naive{{na\"{\i}ve}\xspace}

%Sanjiban and Rahul: Choose your own colors.
\def\rephrasek#1{\textcolor{blue}{#1}}
\def\ssnote#1{\textcolor{red}{#1}}
\def\avknote#1{\textcolor{cyan}{#1}}

\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
%\newtheorem{thm}{Theorem}[section]
\newtheorem{observation}[thm]{Observation}
%\newtheorem{thm}{Theorem}
\newtheorem{cor}{Corollary}
%\newtheorem{def}[thm]{Definition}


%tex tools
\newcommand{\ignore}[1]{}
\newcommand{\first}[2]{#1}
\newcommand{\second}[2]{#2}
%\newcommand{\arxiv}[2]{#2}
%
%\newboolean{ICRA}
%\newboolean{ARXIV}
%
%\setboolean{ICRA}{false}
%\ifthenelse{\boolean{ICRA}}
%	{\setboolean{ARXIV}{false} }
%	{\setboolean{ARXIV}{true}  }
%
%
%\newcommand{\textVersion}[2]
%{\ifthenelse{\boolean{ICRA} }{#1}{}\ifthenelse{\boolean{ARXIV}}{#2}{}}


\def\nbr{\mathop{\mathrm{nbr}}}
\def\prnt{\mathop{\mathrm{p}}}
\def\anc{\mathop{\mathrm{anc}}}
\def\dist{\mathop{\mathrm{dist}}}
\def\cmprs{\ensuremath{\chi}}


\newboolean{ShowAuthors}
\setboolean{ShowAuthors}{false}
\def\blind#1{
\ifthenelse{\boolean {ShowAuthors}}{#1}{}
}

\newcommand{\captionstyle}{\sf \footnotesize }

% Change these to the relevant algorithm names
\newcommand\algname[1]{\textsf{#1}\xspace}
\newcommand\lwastar{\algname{LWA*}}
\newcommand\astar{\algname{A*}}
\newcommand\lazySP{\algname{LazySP}}


